Hgformer: Hyperbolic Graph Transformer for Recommendation

The cold start problem is a challenging problem faced by most modern recommender systems. By leveraging knowledge from other domains, cross-domain recommendation can be an effective method to alleviate the cold start problem. However, the modelling distortion for long-tail data, which is widely present in recommender systems, is often overlooked in cross-domain recommendation. In this research, we propose a hyperbolic manifold based cross-domain collaborative filtering model using BiTGCF as the base model. We introduce the hyperbolic manifold and construct new propagation layer and transfer layer to address these challenges. The significant performance improvements across various datasets compared to the baseline models demonstrate the effectiveness of our proposed model.

==> sections/conclusion.tex <==
\section{Conclusion}
In this study, we proposed a novel hyperbolic graph transformer model called Hgformer to fit the long-tail nature of the data.  
Specifically, we redefined self-attention in the hyperbolic manifold and then reduced the computation complexity to linear. The numerical experiments showed that our proposed model outperformed the previous work.

